AskChart: Universal Chart Understanding through Textual Enhancement

Chart understanding tasks such as ChartQA and Chart-to-Text involve automatically extracting and interpreting key information from charts, enabling users to query or convert visual data into structured formats. State-of-the-art approaches primarily focus on visual cues from chart images, failing to explicitly incorporate rich textual information (e.g., data labels and axis labels) embedded within the charts. This textual information is vital for intuitive human comprehension and interpretation of charts. Moreover, existing models are often large and computationally intensive, limiting their practical applicability. In this paper, we introduce AskChart, a universal model that explicitly integrates both textual and visual cues from charts using a Mixture of Experts (MoE) architecture. AskChart facilitates the learning of enhanced visual-textual representations of charts for effectively handling multiple chart understanding tasks, while maintaining a smaller model size. To capture the synergy between visual and textual modalities, we curate a large-scale dataset named ChartBank with about 7.5M data samples, which helps align textual and visual information and facilitates the extraction of visual entities and text. To effectively train AskChart, we design a three-stage training strategy to align visual and textual modalities for learning robust visual-textual representations and optimizing the learning of the MoE layer. Extensive experiments across five datasets demonstrate the significant performance gains of AskChart in four chart understanding tasks. Remarkably, AskChart with 4.6B parameters outperforms state-of-the-art models with 13B parameters by 68.3% in Open-ended ChartQA and 49.2% in Chart-to-Text tasks, while achieving comparable performance in ChartQA and Chart-to-Table tasks.

==> tables/miniPage-Chart2table.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=0.7\linewidth]{images/appendix_eg/chart2table_1.pdf}
        \vspace{-.5em}
        \caption{Example \#1 for Chart-to-Table tasks.}
        % \label{framework}
        % \vspace{-.3cm}
    \end{minipage}
    \hspace{0.04\linewidth}  % 设置图片之间的间距
    \begin{minipage}{0.45\linewidth}
        % \vspace{-1em}
        \centering
        \includegraphics[width=0.7\linewidth]{images/appendix_eg/chart2table_2.pdf}
        \vspace{-0.5em}
        \caption{Example \#2 for Chart-to-Table tasks.}
        % \label{framework}
    \end{minipage}
\end{figure*}


==> tables/miniPage-Chart2text.tex <==
\begin{figure*}[htbp]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/appendix_eg/chart2txt_1.pdf}
        \vspace{-0.5em}
        \caption{Example \#1 for Chart-to-Text tasks.}
        \label{fig:chart2txt1}
    \end{minipage}
    \hspace{0.04\linewidth}  % 设置图片之间的间距
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/appendix_eg/chart2txt_2.pdf}
        \vspace{-0.5em}
        \caption{Example \#2 for Chart-to-Text tasks.}
        \label{fig:chart2txt2}
    \end{minipage}
\end{figure*}

